Fast Poisson brackets and constraint algebras in canonical gravity

In the study of alternative or extended theories of gravity, Dirac's Hamiltonian constraint algorithm is invaluable for enumerating the propagating modes and gauge symmetries. For gravity, this canonical approach is frequently applied as a means for finding pathologies such as strongly coupled modes; more generally it facilitates the reconstruction of gauge symmetries and the quantization of gauge theories. For gravity, however, the algorithm can become notoriously arduous to implement. We present a simple computer algebra package for efficiently computing Poisson brackets and reconstructing constraint algebras. The tools are stress-tested against pure general relativity and modified gravity, including the order reduction of general relativity at two loops.

==> code_listings_Hamilcar-ComputeSuperHamiltonianAutocommutator.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo

==> code_listings_Hamilcar-ComputeSuperHamiltonianSuperMomentumBracket.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; 

==> code_listings_Hamilcar-ComputeSuperMomentumAutocommutatorContravariant.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; 

==> code_listings_Hamilcar-ComputeSuperMomentumAutocommutatorCovariant.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; 

==> code_listings_Hamilcar-DefineGravitationalCoupling.tex <==
In[#]:= DefConstantSymbol[GravitationalCoupling, PrintAs -> "\[Kappa]"]

==> code_listings_Hamilcar-DefineLapse.tex <==
In[#]:= DefTensor[Lapse[], M3, PrintAs -> "\[ScriptCapitalN]"]

==> code_listings_Hamilcar-DefineScalarSmearingF.tex <==
In[#]:= DefTensor[ScalarSmearingF[], M3, PrintAs -> "\[ScriptF]"]

==> code_listings_Hamilcar-DefineScalarSmearingS.tex <==
In[#]:= DefTensor[ScalarSmearingS[], M3, PrintAs -> "\[ScriptS]"]

==> code_listings_Hamilcar-DefineShift.tex <==
In[#]:= DefTensor[Shift[m], M3, PrintAs -> "\[ScriptCapitalN]"]

==> code_listings_Hamilcar-DefineSuperHamiltonian.tex <==
In[#]:= DefTensor[SuperHamiltonian[], M3, PrintAs -> "\[ScriptCapitalH]"]; FromSuperHamiltonian = MakeRule[{SuperHamiltonian[], (1/((1/GravitationalCoupling^2) * Sqrt[DetG[]])) * (ConjugateMomentumG[i, j] * ConjugateMomentumG[-i, -j] - (1/2) * TraceConjugateMomentumG[]^2) - (1/GravitationalCoupling^2) * Sqrt[DetG[]] * RicciScalarCD[]}, MetricOn -> All, ContractMetrics -> True]

==> code_listings_Hamilcar-DefineSuperMomentum.tex <==
In[#]:= DefTensor[SuperMomentum[-i], M3, PrintAs -> "\[ScriptCapitalH]"]; FromSuperMomentum = MakeRule[{SuperMomentum[-i], -2 * CD[-j][ConjugateMomentumG[j, -i]]}, MetricOn -> All, ContractMetrics -> True]

==> code_listings_Hamilcar-DefineVectorSmearingContravariantF.tex <==
In[#]:= DefTensor[VectorSmearingContravariantF[i], M3, PrintAs -> "\[ScriptF]"]

==> code_listings_Hamilcar-DefineVectorSmearingContravariantS.tex <==
In[#]:= DefTensor[VectorSmearingContravariantS[i], M3, PrintAs -> "\[ScriptS]"]

==> code_listings_Hamilcar-DefineVectorSmearingCovariantF.tex <==
In[#]:= DefTensor[VectorSmearingCovariantF[-i], M3, PrintAs -> "\[ScriptF]"]

==> code_listings_Hamilcar-DefineVectorSmearingCovariantS.tex <==
In[#]:= DefTensor[VectorSmearingCovariantS[-i], M3, PrintAs -> "\[ScriptS]"]

==> code_listings_Hamilcar-EnableManualSmearing.tex <==
In[#]:= $ManualSmearing = True

==> code_listings_Hamilcar-FindAlgebraSuperHamiltonianAutocommutator.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{SuperMomentum}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Constraints -> {SuperMomentum[i]}, Method -> Solve, Verify -> True] & ; 

==> code_listings_Hamilcar-FindAlgebraSuperHamiltonianSuperMomentumBracket.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{SuperHamiltonian}, {CD, ScalarSmearingF, VectorSmearingContravariantS}}}, Constraints -> {SuperHamiltonian[]}, Method -> Solve, Verify -> True] & ; 

==> code_listings_Hamilcar-FindAlgebraSuperMomentumAutocommutatorContravariant.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{SuperMomentum}, {CD, VectorSmearingContravariantF, VectorSmearingContravariantS}}}, Constraints -> {SuperMomentum[i]}, Method -> Solve, Verify -> True] & ; 

==> code_listings_Hamilcar-FindAlgebraSuperMomentumAutocommutatorCovariant.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{SuperMomentum}, {CD, VectorSmearingCovariantF, VectorSmearingCovariantS}}}, Constraints -> {SuperMomentum[i]}, Method -> Solve, Verify -> True] & ; 

==> code_listings_Hamilcar-PrependTotalFromSuperHamiltonian.tex <==
In[#]:= PrependTotalFrom[FromSuperHamiltonian]

==> code_listings_Hamilcar-PrependTotalFromSuperMomentum.tex <==
In[#]:= PrependTotalFrom[FromSuperMomentum]

==> code_listings_Hamilcar-PrependTotalFromTraceConjugateMomentumG.tex <==
In[#]:= PrependTotalFrom[FromTraceConjugateMomentumG]

==> code_listings_Hamilcar-SetupSuperHamiltonianAutocommutator.tex <==
In[#]:= Expr = {ScalarSmearingF[] * SuperHamiltonian[], ScalarSmearingS[] * SuperHamiltonian[]}

==> code_listings_Hamilcar-SetupSuperHamiltonianSuperMomentumBracket.tex <==
In[#]:= Expr = {ScalarSmearingF[] * SuperHamiltonian[], VectorSmearingContravariantS[i] * SuperMomentum[-i]}

==> code_listings_Hamilcar-SetupSuperMomentumAutocommutatorContravariant.tex <==
In[#]:= Expr = {VectorSmearingContravariantF[i] * SuperMomentum[-i], VectorSmearingContravariantS[j] * SuperMomentum[-j]}

==> code_listings_Hamilcar-SetupSuperMomentumAutocommutatorCovariant.tex <==
In[#]:= Expr = {VectorSmearingCovariantF[-i] * SuperMomentum[i], VectorSmearingCovariantS[-j] * SuperMomentum[j]}

==> code_listings_Hamilcar-TraceConjugateMomentumG.tex <==
In[#]:= DefTensor[TraceConjugateMomentumG[], M3, PrintAs -> "\[Pi]"]; FromTraceConjugateMomentumG = MakeRule[{TraceConjugateMomentumG[], Scalar[ConjugateMomentumG[a, -a]]}, MetricOn -> All, ContractMetrics -> True]

==> code_listings_LoadHamilcar.tex <==
In[#]:= Get["xAct`Hamilcar`"];


==> code_listings_Private-ComputeEquationOfMotionConjugateMomentumExtrinsicCurvature.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= VarD[TensorSmearingCovariantF[-i, -j], CD]; Expr //= TotalFrom; Expr //= #1 /. ToPrimaryShell & ; Expr //= TotalTo; 

==> code_listings_Private-ComputeEquationOfMotionConjugateMomentumG.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= VarD[TensorSmearingCovariantF[-i, -j], CD]; Expr //= TotalFrom; Expr //= #1 /. ToPrimaryShell & ; Expr //= TotalTo; 

==> code_listings_Private-ComputeEquationOfMotionExtrinsicCurvature.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= VarD[TensorSmearingContravariantF[i, j], CD]; Expr //= TotalFrom; Expr //= #1 /. ToPrimaryShell & ; Expr //= TotalTo; 

==> code_listings_Private-ComputeEquationOfMotionG.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= VarD[TensorSmearingContravariantF[i, j], CD]; Expr //= TotalFrom; Expr //= TotalTo; 

==> code_listings_Private-ComputePoissonBracketExtrinsicCurvature.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> False] & ) @@ #1 & ; Expr //= FullSimplify; 

==> code_listings_Private-ComputePrimaryConstraintSuperHamiltonian.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; 

==> code_listings_Private-ComputePrimaryConstraintSuperMomentum.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; 

==> code_listings_Private-ComputeSecondaryConstraintPrimaryConstraint.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= #1 /. ToPrimaryShellExplicit & ; Expr //= ToCanonical; Expr //= ContractMetric; Expr //= ScreenDollarIndices; Expr //= FullSimplify; 

==> code_listings_Private-ComputeSuperHamiltonianSuperHamiltonian.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= FullSimplify; 

==> code_listings_Private-ComputeSuperHamiltonianSuperMomentum.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= FullSimplify; 

==> code_listings_Private-ComputeSuperMomentumSuperMomentum.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; Expr //= TotalTo; Expr //= FullSimplify; 

==> code_listings_Private-DefineExtrinsicCurvature.tex <==
In[#]:= DefCanonicalField[ExtrinsicCurvature[-m, -n], Symmetric[{-m, -n}], FieldSymbol -> "\[ScriptCapitalK]", MomentumSymbol -> "\[Rho]"]; 

==> code_listings_Private-DefinePrimaryConstraint.tex <==
In[#]:= DefTensor[PrimaryConstraint[i, j], M3, Symmetric[{i, j}], PrintAs -> "\[CapitalPhi]"]; AutomaticRules[PrimaryConstraint, MakeRule[{PrimaryConstraint[i, -i], 0}, MetricOn -> All, ContractMetrics -> True]]; FromPrimaryConstraint = MakeRule[{PrimaryConstraint[i, j], ConjugateMomentumExtrinsicCurvature[i, j] - (1/3) * G[i, j] * TraceConjugateMomentumExtrinsicCurvature[]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromPrimaryConstraint]; 

==> code_listings_Private-DefineSecondaryConstraint.tex <==
In[#]:= DefTensor[SecondaryConstraint[i, j], M3, Symmetric[{i, j}], PrintAs -> "\[CapitalPsi]"]; AutomaticRules[SecondaryConstraint, MakeRule[{SecondaryConstraint[i, -i], 0}, MetricOn -> All, ContractMetrics -> True]]; FromSecondaryConstraint = MakeRule[{SecondaryConstraint[i, j], Evaluate[Expr]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromSecondaryConstraint]; 

==> code_listings_Private-DefineSuperHamiltonian.tex <==
In[#]:= DefTensor[SuperHamiltonian[], M3, PrintAs -> "\[ScriptCapitalH]"]; FromSuperHamiltonian = MakeRule[{SuperHamiltonian[], (1/(144 * Sqrt[DetG[]])) * TraceConjugateMomentumExtrinsicCurvature[]^2 - 2 * ConjugateMomentumG[m, n] * ExtrinsicCurvature[-m, -n] + (1/6) * TraceConjugateMomentumExtrinsicCurvature[] * (TraceExtrinsicCurvature[]^2 - 3 * ExtrinsicCurvature[-m, -n] * ExtrinsicCurvature[m, n] + RicciScalarCD[]) - (Sqrt[DetG[]]/3) * CD[-m][CD[m][TraceConjugateMomentumExtrinsicCurvature[]/Sqrt[DetG[]]]]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromSuperHamiltonian]; 

==> code_listings_Private-DefineSuperMomentum.tex <==
In[#]:= DefTensor[SuperMomentum[-m], M3, PrintAs -> "\[ScriptCapitalH]"]; FromSuperMomentum = MakeRule[{SuperMomentum[-m], (1/3) * TraceConjugateMomentumExtrinsicCurvature[] * CD[-m][TraceExtrinsicCurvature[]] - 2 * Sqrt[DetG[]] * CD[-n][(3 * ConjugateMomentumG[-m, n] + TraceConjugateMomentumExtrinsicCurvature[] * ExtrinsicCurvature[-m, n])/(3 * Sqrt[DetG[]])]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromSuperMomentum]; 

==> code_listings_Private-DefineTensorSmearing.tex <==
In[#]:= DefTensor[TensorSmearingCovariantS[-i, -j], M3, Symmetric[{-i, -j}], PrintAs -> "\[ScriptS]"]; DefTensor[TensorSmearingContravariantS[i, j], M3, Symmetric[{i, j}], PrintAs -> "\[ScriptS]"]; DefTensor[TensorSmearingCovariantF[-i, -j], M3, Symmetric[{-i, -j}], PrintAs -> "\[ScriptF]"]; DefTensor[TensorSmearingContravariantF[i, j], M3, Symmetric[{i, j}], PrintAs -> "\[ScriptF]"]; 

==> code_listings_Private-DefineToPrimaryShell.tex <==
In[#]:= ToPrimaryShell = MakeRule[{ConjugateMomentumExtrinsicCurvature[i, j], (1/3) * G[i, j] * TraceConjugateMomentumExtrinsicCurvature[]}, MetricOn -> All, ContractMetrics -> True]; 

==> code_listings_Private-DefineToPrimaryShellExplicit.tex <==
In[#]:= ToPrimaryShellExplicit = MakeRule[{ConjugateMomentumExtrinsicCurvature[i, j], (1/3) * G[i, j] * TraceConjugateMomentumExtrinsicCurvature[] + PrimaryConstraint[i, j]}, MetricOn -> All, ContractMetrics -> True]; 

==> code_listings_Private-DefineTotalHamiltonian.tex <==
In[#]:= DefTensor[TotalHamiltonian[], M3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptCapitalH]\),\(T\)]\)"]; FromTotalHamiltonian = MakeRule[{TotalHamiltonian[], Lapse[] * SuperHamiltonian[] + Shift[m] * SuperMomentum[-m] + Lapse[] * Multiplier[-i, -j] * PrimaryConstraint[i, j]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromTotalHamiltonian]; 

==> code_listings_Private-DefineTraceConjugateMomentumExtrinsicCurvature.tex <==
In[#]:= DefTensor[TraceConjugateMomentumExtrinsicCurvature[], M3, PrintAs -> "\[Rho]"]; FromTraceConjugateMomentumExtrinsicCurvature = MakeRule[{TraceConjugateMomentumExtrinsicCurvature[], Scalar[ConjugateMomentumExtrinsicCurvature[a, -a]]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromTraceConjugateMomentumExtrinsicCurvature]; ToTraceConjugateMomentumExtrinsicCurvature = MakeRule[{ConjugateMomentumExtrinsicCurvature[a, -a], TraceConjugateMomentumExtrinsicCurvature[]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalTo[ToTraceConjugateMomentumExtrinsicCurvature]; 

==> code_listings_Private-DefineTraceExtrinsicCurvature.tex <==
In[#]:= DefTensor[TraceExtrinsicCurvature[], M3, PrintAs -> "\[ScriptCapitalK]"]; FromTraceExtrinsicCurvature = MakeRule[{TraceExtrinsicCurvature[], Scalar[ExtrinsicCurvature[a, -a]]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromTraceExtrinsicCurvature]; ToTraceExtrinsicCurvature = MakeRule[{ExtrinsicCurvature[a, -a], TraceExtrinsicCurvature[]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalTo[ToTraceExtrinsicCurvature]; 

==> code_listings_Private-FindAlgebraPrimaryConstraintSuperHamiltonian.tex <==
In[#]:= Expr //= TotalFrom; Expr //= FindAlgebra[#1, {{{SecondaryConstraint, TensorSmearingCovariantF, ScalarSmearingS}}, {{PrimaryConstraint, ExtrinsicCurvature, TensorSmearingCovariantF, ScalarSmearingS}}}, Constraints -> {PrimaryConstraint[i, j], SecondaryConstraint[i, j]}, Method -> Solve, Verify -> False] & ; 

==> code_listings_Private-FindAlgebraPrimaryConstraintSuperMomentum.tex <==
In[#]:= Expr //= TotalFrom; Expr //= FindAlgebra[#1, {{{PrimaryConstraint}, {CD, TensorSmearingCovariantF, VectorSmearingCovariantS}}}, Constraints -> {SuperHamiltonian[], SuperMomentum[i], PrimaryConstraint[i, j], SecondaryConstraint[i, j]}, Method -> Solve, Verify -> False] & ; 

==> code_listings_Private-FindAlgebraSuperHamiltonianSuperHamiltonian.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{PrimaryConstraint, ExtrinsicCurvature}, {CD, CD, ScalarSmearingF, ScalarSmearingS}}, {{SuperMomentum}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{SecondaryConstraint}, {CD, CD, ScalarSmearingF, ScalarSmearingS}}}, Constraints -> {SuperHamiltonian[], SuperMomentum[i], PrimaryConstraint[i, j], SecondaryConstraint[i, j]}, Method -> Solve, Verify -> False] & ; 

==> code_listings_Private-FindAlgebraSuperHamiltonianSuperMomentum.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{PrimaryConstraint}, {CD, CD, CD, ScalarSmearingF, VectorSmearingCovariantS}}, {{PrimaryConstraint, RicciCD}, {CD, ScalarSmearingF, VectorSmearingCovariantS}}, {{PrimaryConstraint, ConjugateMomentumExtrinsicCurvature}, {CD, ScalarSmearingF, VectorSmearingCovariantS}}, {{PrimaryConstraint}, {CD, ExtrinsicCurvature, ExtrinsicCurvature, ScalarSmearingF, VectorSmearingCovariantS}}, {{SecondaryConstraint}, {CD, ExtrinsicCurvature, ScalarSmearingF, VectorSmearingCovariantS}}, {{SuperMomentum, ExtrinsicCurvature, ScalarSmearingF, VectorSmearingCovariantS}}, {{SuperHamiltonian}, {CD, ScalarSmearingF, VectorSmearingCovariantS}}}, Constraints -> {SuperHamiltonian[], SuperMomentum[i], PrimaryConstraint[i, j], SecondaryConstraint[i, j]}, Method -> Solve, DDIs -> False, Verify -> False] & ; 

==> code_listings_Private-FindAlgebraSuperMomentumSuperMomentum.tex <==
In[#]:= Expr //= FindAlgebra[#1, {{{PrimaryConstraint}, {CD, CD, ExtrinsicCurvature, VectorSmearingCovariantF, VectorSmearingCovariantS}}, {{SecondaryConstraint}, {CD, CD, VectorSmearingCovariantF, VectorSmearingCovariantS}}, {{SuperMomentum}, {CD, VectorSmearingCovariantF, VectorSmearingCovariantS}}}, Constraints -> {SuperHamiltonian[], SuperMomentum[i], PrimaryConstraint[i, j], SecondaryConstraint[i, j]}, Method -> Solve, Verify -> False] & ; 

==> code_listings_Private-SetupEquationOfMotionConjugateMomentumExtrinsicCurvature.tex <==
In[#]:= Expr = {TensorSmearingCovariantF[-i, -j] * ConjugateMomentumExtrinsicCurvature[i, j], TotalHamiltonian[]}; 

==> code_listings_Private-SetupEquationOfMotionConjugateMomentumG.tex <==
In[#]:= Expr = {TensorSmearingCovariantF[-i, -j] * ConjugateMomentumG[i, j], TotalHamiltonian[]}; 

==> code_listings_Private-SetupEquationOfMotionExtrinsicCurvature.tex <==
In[#]:= Expr = {TensorSmearingContravariantF[i, j] * ExtrinsicCurvature[-i, -j], TotalHamiltonian[]}; 

==> code_listings_Private-SetupEquationOfMotionG.tex <==
In[#]:= Expr = {TensorSmearingContravariantF[i, j] * G[-i, -j], TotalHamiltonian[]}; 

==> code_listings_Private-SetupPoissonBracketExtrinsicCurvature.tex <==
In[#]:= Expr = {ExtrinsicCurvature[-m, -n], ConjugateMomentumExtrinsicCurvature[a, b]}; 

==> code_listings_Private-SetupPrimaryConstraintSuperHamiltonian.tex <==
In[#]:= Expr = {TensorSmearingCovariantF[-i, -j] * PrimaryConstraint[i, j], ScalarSmearingS[] * SuperHamiltonian[]}; 

==> code_listings_Private-SetupPrimaryConstraintSuperMomentum.tex <==
In[#]:= Expr = {TensorSmearingCovariantF[-i, -j] * PrimaryConstraint[i, j], VectorSmearingCovariantS[-j] * SuperMomentum[j]}; 

==> code_listings_Private-SetupSecondaryConstraintPrimaryConstraint.tex <==
In[#]:= Expr = {TensorSmearingCovariantF[-i, -j] * SecondaryConstraint[i, j], TensorSmearingCovariantS[-k, -l] * PrimaryConstraint[k, l]}; 

==> code_listings_Private-SetupSuperHamiltonianSuperHamiltonian.tex <==
In[#]:= Expr = {ScalarSmearingF[] * SuperHamiltonian[], ScalarSmearingS[] * SuperHamiltonian[]}; 

==> code_listings_Private-SetupSuperHamiltonianSuperMomentum.tex <==
In[#]:= Expr = {ScalarSmearingF[] * SuperHamiltonian[], VectorSmearingCovariantS[i] * SuperMomentum[-i]}; 

==> code_listings_Private-SetupSuperMomentumSuperMomentum.tex <==
In[#]:= Expr = {VectorSmearingCovariantF[-i] * SuperMomentum[i], VectorSmearingCovariantS[-j] * SuperMomentum[j]}; 

==> code_listings_ReproductionOfResults-CombineBrackets.tex <==
In[#]:= Expr = OrderUnityBracketValue + CrossBracket01Value + CrossBracket10Value; Expr //= StandardSimplify; BracketKValue = Expr; 

==> code_listings_ReproductionOfResults-ComputeCrossBracket01.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; CrossBracket01Value = Expr; 

==> code_listings_ReproductionOfResults-ComputeCrossBracket10.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; CrossBracket10Value = Expr; 

==> code_listings_ReproductionOfResults-ComputeOrderUnityBracket.tex <==
In[#]:= Expr //= (PoissonBracket[#1, #2, Parallel -> True] & ) @@ #1 & ; OrderUnityBracketValue = Expr; 

==> code_listings_ReproductionOfResults-DefineCosmologicalConstant.tex <==
In[#]:= DefConstantSymbol[CosmologicalConstant, PrintAs -> "\[CapitalLambda]"]; 

==> code_listings_ReproductionOfResults-DefineExtractBracketAnatomy.tex <==
In[#]:= Options[ExtractBracketAnatomy] = {CosmologicalConstantOrder -> All, WilsonCoefficientOrder -> All}; ExtractBracketAnatomy[OptionsPattern[]] := Module[{Expr = BracketKValue}, If[ !OptionValue[CosmologicalConstantOrder] === All, Expr //= Series[#1, {CosmologicalConstant, 0, 10}] & ; Expr //= Normal; Expr = (Coefficient[Expr, CosmologicalConstant, #1] * CosmologicalConstant^#1 & ) /@ OptionValue[CosmologicalConstantOrder]; Expr //= Total; ]; If[ !OptionValue[WilsonCoefficientOrder] === All, Expr //= Series[#1, {WilsonCoefficientOrder, 0, 10}] & ; Expr //= Normal; Expr = (Coefficient[Expr, WilsonCoefficient, #1] * WilsonCoefficient^#1 & ) /@ OptionValue[WilsonCoefficientOrder]; Expr //= Total; ]; Expr //= StandardSimplify; Expr]; 

==> code_listings_ReproductionOfResults-DefineReducedHamiltonianConstraint.tex <==
In[#]:= DefTensor[ReducedHamiltonianConstraint[], M3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptCapitalH]\),\(red\)]\)"]; FromReducedHamiltonianConstraint = MakeRule[{ReducedHamiltonianConstraint[], Sqrt[DetG[]] * (-(TraceScriptQ[] - 2 * CosmologicalConstant)/EinsteinConstant^2 + 8 * WilsonCoefficient * EinsteinConstant^2 * ScriptQSingleContraction[i, -j] * (2 * ScriptQSingleContraction[j, -k] * ScriptQSingleContraction[k, -i] - 3 * ScriptL[j, -k, -l] * ScriptL[-i, k, l]) - 24 * WilsonCoefficient * EinsteinConstant^2 * CosmologicalConstant * (2 * ScriptQSingleContraction[i, -j] * ScriptQSingleContraction[j, -i] - 2 * CosmologicalConstant^2 - ScriptL[-k, i, j] * ScriptL[k, -i, -j]))}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromReducedHamiltonianConstraint]; 

==> code_listings_ReproductionOfResults-DefineReducedHamiltonianOrderUnity.tex <==
In[#]:= DefTensor[ReducedHamiltonianOrderUnity[], M3, PrintAs -> "\!\(\ * SubscriptBox[\(\ * OverscriptBox[\(\[ScriptCapitalH]\),\((0)\)]\),\(red\)]\)"]; Expr = ReducedHamiltonianConstraint[]; Expr //= #1 /. FromReducedHamiltonianConstraint & ; Expr //= Coefficient[#1, WilsonCoefficient, 0] & ; FromReducedHamiltonianOrderUnity = MakeRule[{ReducedHamiltonianOrderUnity[], Evaluate[Expr]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromReducedHamiltonianOrderUnity]; 

==> code_listings_ReproductionOfResults-DefineReducedHamiltonianOrderWilsonCoefficient.tex <==
In[#]:= DefTensor[ReducedHamiltonianOrderWilsonCoefficient[], M3, PrintAs -> "\!\(\ * SubscriptBox[\(\ * OverscriptBox[\(\[ScriptCapitalH]\),\((1)\)]\),\(red\)]\)"]; Expr = ReducedHamiltonianConstraint[]; Expr //= #1 /. FromReducedHamiltonianConstraint & ; Expr //= Coefficient[#1, WilsonCoefficient, 1] & ; Expr  * = WilsonCoefficient; FromReducedHamiltonianOrderWilsonCoefficient = MakeRule[{ReducedHamiltonianOrderWilsonCoefficient[], Evaluate[Expr]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromReducedHamiltonianOrderWilsonCoefficient]; 

==> code_listings_ReproductionOfResults-DefineReducedMomentumConstraint.tex <==
In[#]:= DefTensor[ReducedMomentumConstraint[i], M3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptCapitalH]\),\(red\)]\)"]; FromReducedMomentumConstraint = MakeRule[{ReducedMomentumConstraint[i], Sqrt[DetG[]] * (-2 * (ScriptLContraction[i]/EinsteinConstant^2))}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromReducedMomentumConstraint]; 

==> code_listings_ReproductionOfResults-DefineScriptK.tex <==
In[#]:= DefTensor[ScriptK[-i, -j], M3, Symmetric[{-i, -j}], PrintAs -> "\[GothicCapitalK]"]; FromScriptK = MakeRule[{ScriptK[-i, -j], (-EinsteinConstant^2) * (ConjugateMomentumG[-i, -j]/Sqrt[DetG[]] - (G[-i, -j]/2) * (TraceConjugateMomentumG[]/Sqrt[DetG[]]))}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromScriptK]; 

==> code_listings_ReproductionOfResults-DefineScriptL.tex <==
In[#]:= DefTensor[ScriptL[i, -j, -k], M3, Antisymmetric[{-j, -k}], PrintAs -> "\[GothicCapitalL]"]; FromScriptL = MakeRule[{ScriptL[i, -j, -k], CD[-k][ScriptK[-j, i]] - CD[-j][ScriptK[-k, i]]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromScriptL]; 

==> code_listings_ReproductionOfResults-DefineScriptLContraction.tex <==
In[#]:= DefTensor[ScriptLContraction[-i], M3, PrintAs -> "\[GothicCapitalL]"]; FromScriptLContraction = MakeRule[{ScriptLContraction[-i], ScriptL[j, -j, -i]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromScriptLContraction]; 

==> code_listings_ReproductionOfResults-DefineScriptQ.tex <==
In[#]:= DefTensor[ScriptQ[i, j, -k, -l], M3, {Antisymmetric[{i, j}], Antisymmetric[{-k, -l}]}, PrintAs -> "\[GothicCapitalQ]"]; FromScriptQ = MakeRule[{ScriptQ[i, j, -k, -l], ScriptK[i, -k] * ScriptK[j, -l] - ScriptK[i, -l] * ScriptK[j, -k] + RiemannCD[i, j, -k, -l]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromScriptQ]; 

==> code_listings_ReproductionOfResults-DefineScriptQSingleContraction.tex <==
In[#]:= DefTensor[ScriptQSingleContraction[-i, -j], M3, Symmetric[{-i, -j}], PrintAs -> "\[GothicCapitalQ]"]; FromScriptQSingleContraction = MakeRule[{ScriptQSingleContraction[i, -j], ScriptQ[i, k, -j, -k]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromScriptQSingleContraction]; 

==> code_listings_ReproductionOfResults-DefineStandardSimplify.tex <==
In[#]:= StandardSimplify[Expr_] := Module[{Result = Expr}, Result //= ToCanonical; Result //= ContractMetric; Result //= ScreenDollarIndices; Result //= CollectTensors; Result]; 

==> code_listings_ReproductionOfResults-DefineTraceScriptK.tex <==
In[#]:= DefTensor[TraceScriptK[], M3, PrintAs -> "\[GothicCapitalK]"]; FromTraceScriptK = MakeRule[{TraceScriptK[], G[i, j] * ScriptK[-i, -j]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromTraceScriptK]; 

==> code_listings_ReproductionOfResults-DefineTraceScriptQ.tex <==
In[#]:= DefTensor[TraceScriptQ[], M3, PrintAs -> "\[GothicCapitalQ]"]; FromTraceScriptQ = MakeRule[{TraceScriptQ[], ScriptQ[i, j, -i, -j]}, MetricOn -> All, ContractMetrics -> True]; PrependTotalFrom[FromTraceScriptQ]; 

==> code_listings_ReproductionOfResults-DefineWilsonCoefficient.tex <==
In[#]:= DefConstantSymbol[WilsonCoefficient, PrintAs -> "\[Alpha]"]; 

==> code_listings_ReproductionOfResults-ExtractFirstOrderBracket.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {1}, WilsonCoefficientOrder -> All]; 

==> code_listings_ReproductionOfResults-ExtractSecondOrderBracket.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {2}, WilsonCoefficientOrder -> All]; 

==> code_listings_ReproductionOfResults-ExtractZerothOrderBracket.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {0}, WilsonCoefficientOrder -> All]; 

==> code_listings_ReproductionOfResults-FindAlgebraFirstOrder.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {1}, WilsonCoefficientOrder -> All]; Expr //= FindAlgebra[#1, {{{ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ScriptQSingleContraction}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, CD, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{RicciCD, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{RicciScalarCD, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Method -> Solve, Verify -> True, DDIs -> True] & ; 

==> code_listings_ReproductionOfResults-FindAlgebraSecondOrder.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {2}, WilsonCoefficientOrder -> All]; Expr //= FindAlgebra[#1, {{{ReducedMomentumConstraint}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ReducedHamiltonianOrderUnity}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptQSingleContraction, ReducedMomentumConstraint}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, CD, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{RicciCD, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Constraints -> {ReducedMomentumConstraint[i], ReducedHamiltonianOrderUnity[]}, Method -> Solve, Verify -> True] & ; 

==> code_listings_ReproductionOfResults-FindAlgebraZerothOrderA.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {0}, WilsonCoefficientOrder -> All]; Expr //= FindAlgebra[#1, {{{CD, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, ScriptK}, {RicciCD, RicciCD}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, ScriptK}, {CD, ScriptK}, {CD, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, ScriptK}, {RicciCD, ScriptK, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{CD, ScriptK}, {ScriptK, ScriptK, ScriptK, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Method -> Solve, Verify -> False] & ; 

==> code_listings_ReproductionOfResults-FindAlgebraZerothOrderB.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {0}, WilsonCoefficientOrder -> All]; Expr //= FindAlgebra[#1, {{{ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ScriptL, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, RicciCD, ScriptK, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ScriptK, ScriptK, ScriptK, ScriptK}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, RicciCD, RicciCD}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Method -> Solve, Verify -> False] & ; 

==> code_listings_ReproductionOfResults-FindAlgebraZerothOrderC.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {0}, WilsonCoefficientOrder -> All]; EinsteinConstant = 1; CosmologicalConstant = 1; WilsonCoefficient = 1; Expr //= FindAlgebra[#1, {{{ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ScriptL, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ScriptL, ScriptQSingleContraction, ScriptQSingleContraction}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Method -> Solve, Verify -> False, DDIs -> True] & ; 

==> code_listings_ReproductionOfResults-FindAlgebraZerothOrderD.tex <==
In[#]:= Expr = ExtractBracketAnatomy[CosmologicalConstantOrder -> {0}, WilsonCoefficientOrder -> All]; Block[{CosmologicalConstant = 0}, Expr //= FindAlgebra[#1, {{{ReducedMomentumConstraint}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ReducedMomentumConstraint, ScriptL, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ReducedMomentumConstraint, ScriptQSingleContraction, ScriptQSingleContraction}, {CD, ScalarSmearingF, ScalarSmearingS}}, {{ReducedHamiltonianOrderUnity, ScriptQSingleContraction, ScriptL}, {CD, ScalarSmearingF, ScalarSmearingS}}}, Constraints -> {ReducedMomentumConstraint[i], ReducedHamiltonianOrderUnity[]}, Method -> Solve, Verify -> False] & ; ]; 

==> code_listings_ReproductionOfResults-SetupCrossBracket01.tex <==
In[#]:= Expr = {ScalarSmearingF[] * ReducedHamiltonianOrderUnity[], ScalarSmearingS[] * ReducedHamiltonianOrderWilsonCoefficient[]}; 

==> code_listings_ReproductionOfResults-SetupCrossBracket10.tex <==
In[#]:= Expr = {ScalarSmearingF[] * ReducedHamiltonianOrderWilsonCoefficient[], ScalarSmearingS[] * ReducedHamiltonianOrderUnity[]}; 

==> code_listings_ReproductionOfResults-SetupOrderUnityBracket.tex <==
In[#]:= Expr = {ScalarSmearingF[] * ReducedHamiltonianOrderUnity[], ScalarSmearingS[] * ReducedHamiltonianOrderUnity[]}; 
